Class Model Generation from Requirements using Large Language Models

The emergence of Large Language Models (LLMs) has opened new opportunities to automate software engineering activities that traditionally require substantial manual effort. Among these, class diagram generation represents a critical yet resource-intensive phase in software design. This paper investigates the capabilities of state-of-the-art LLMs, including GPT-5, Claude Sonnet 4.0, Gemini 2.5 Flash Thinking, and Llama-3.1-8B-Instruct, to generate UML class diagrams from natural language requirements automatically. To evaluate the effectiveness and reliability of LLM-based model generation, we propose a comprehensive dual-validation framework that integrates an LLM-as-a-Judge methodology with human-in-the-loop assessment. Using eight heterogeneous datasets, we apply chain-of-thought prompting to extract domain entities, attributes, and associations, generating corresponding PlantUML representations. The resulting models are evaluated across five quality dimensions: completeness, correctness, conformance to standards, comprehensibility, and terminological alignment. Two independent LLM judges (Grok and Mistral) perform structured pairwise comparisons, and their judgments are further validated against expert evaluations. Our results demonstrate that LLMs can generate structurally coherent and semantically meaningful UML diagrams, achieving substantial alignment with human evaluators. The consistency observed between LLM-based and human-based assessments highlights the potential of LLMs not only as modeling assistants but also as reliable evaluators in automated requirements engineering workflows, offering practical insights into the capabilities and limitations of LLM-driven UML class diagram automation.

==> source/discussion.tex <==
%\vspace*{-.8em}
\section{Discussion}
\label{sec:discussion}

% In the following, we discuss our findings, and speculate on possible solutions to the identified problems. 

In the following, we delve deeper into the discussion of the results, report on additional analyses and discuss any open future opportunities of the LLMs application in UML generation and evaluation.

% discuss results tables 

% This study aimed to identify the most effective LLM for generating UML class diagrams and to assess the quality and consistency of its outputs across eight datasets. The results demonstrate strong correlations in most cases for the GPT-5 model, indicating that the model preserves stable performance across diverse domains.

% The findings of this study have important implications for evaluating LLM models in SE contexts, particularly in assessing their reliability for structured design tasks such as UML diagram generation. 

% rq1: the best llm model

% spearman correlation graph
% \begin{figure}[!ht]
%     \centering
%     \includegraphics[width=1.0\linewidth, height=0.2\textheight]{sections/spearman graph.png}
%     \caption{Spearman Rank Correlation Between Grok and Mistral Judge}
%     \label{fig:spearman}
% \end{figure}

% The results demonstrate strong correlations in most cases for the GPT-5 model, indicating that the model preserves stable performance across diverse domains.
% Similarly, the analysis of RQ1 demonstrates a strong degree of consistency between 2 external model judges (Grok and Mistral) across most datasets, with Spearman correlation values ($\rho$) ranging between 0.8 to 1.0 in 7 out of 8 datasets shown in Table \ref{tab:spearman}. Fig. 1. shows the correlation analysis across 8 datasets further substantiates the high level of agreement between the two evaluation models. This strong agreement particularly in datasets such as Inventory and autopilot reinforces the reliability of LLM-based evaluation frameworks in ranking model-generated UML class diagrams across diverse domains, indicating stable relative ranking performance among the models. 
% possible issues res and solutions to improve res in future

% However, the notably weaker correlation observed in the Pacemaker dataset ($\rho$=0.2) highlights an important outlier. This discrepancy may stem from the dataset's unique domain complexity or differences in how each judge interprets the diagram semantics, despite being guided by standardised evaluation criteria. 

% This insight emphasises the importance of hybrid evaluation strategies, combining automated consistency with human expertise, especially in complex SE tasks to improve robustness across diverse UML design challenges. 

% Examining the model rankings in detail, GPT-5 and Claude models consistently achieved a high position across most datasets, whereas Llama and Gemini generally ranked lower. This pattern suggests that certain LLM architectures in capturing structural and semantic conventions required for UML diagram generation. The consistency in top-performing models reinforces the reliability of the evaluation frameworks, but the variation observed in datasets such as Pacemaker also indicates that model effectiveness can be sensitive to dataset-specific features. 

% Beyond evaluating individual model performance, these findings highlight broader considerations for LLM-based evaluation in SE. The high agreement across most datasets suggests that the automated evaluation can reduce reliance on human judgement, improving efficiency and scalability. Meanwhile, the lower correlation in domain-specific datasets underscores the importance of incorporating context-aware evaluation, either through hybrid human-AI frameworks or train model with more domain knowledge to improve robustness across diverse UML design challenges. Future research could explore strategies to enhance LLMs' generalization across specialized UML tasks and assess the applicability of these methods to other UML model diagrams. 

% rq2: quality of diagram of the best model
% need to relate results back to previous study

% cohen kappa score between LLM-as-a-Judge graph
\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.75\linewidth]{sections/vertical cohen LLM judge.png}
    \caption{Stacked bar charts of the agreement levels between Grok and Mistral across five criteria evaluation}
    \label{fig:LLM}
\end{figure}

% cohen kappa score between evaluators graph
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.75\linewidth]{sections/vertical cohen kappa graph.png}
    \caption{Stacked bar charts of the agreement levels between Evaluators A1 and A2 across five criteria evaluation}
    \label{fig:evaluators}
\end{figure}

Using the results from RQ2 and RQ3, we further explore the quality of the generated model diagrams for the best LLM model chosen, GPT-5. We focused specifically on the degree of agreement among both human evaluators (A1 and A2) and LLM judges (Grok and Mistral). Figs. 2. and 3 show the stacked bar charts showing the measures of agreement across different criteria evaluation using binary classification of Cohen's Kappa. In order to produce these stacked bar charts, we aggregated the total number of each agreement score (1-5) for each criterion, separately for both human evaluators and LLM judges. 

The analysis of agreement scores reveals that both LLM judges (Grok and Mistral) and human evaluators (A1 and A2) demonstrate generally high consistency across most evaluation criteria. In Fig. 2, we observe that Terminological Alignment criteria exhibits high consistency, with Grok assigning a score of 5 and Mistral assigning 4 across all eight datasets, indicating that both models reliably assess terminology use. In contrast, criteria such as Completeness and Correctness show more variation, particularly for Grok, which may reflect differences in how the models' interpret diagram semantics despite using standardised evaluation criteria rubrics. Human evaluators also exhibit strong agreement across most criteria, particularly in Correctness and Understandability, which appear less subjective. Slight variations are observed in criteria such as Completeness and Terminological Alignment, reflecting the inherently subjective nature of these criteria. 

Additionally, the comparison between LLM judges and human evaluators reveals a generally strong alignment in terms of absolute scores across the evaluated criteria as presented in Tables \ref{tab:stats-cohend} and \ref{tab:stats-cohend-HITL}. Both LLMs and humans assigned the highest ratings to terminology and understanding, with identical mean scores for the latter, indicating a shared recognition of clarity and correct use of domain-specific terms. Minor differences were observed in completeness, correctness, and standards, where LLM judges tended to assign slightly higher scores than human evaluators. These minor differences shows that LLMs may over-rank the significance of certain criteria relative to humans, but it sill implies that the reliabilty of LLM in evaluation in as the scoring of LLM mostly aligned with human evaluators. The Kappa values of LLM judges ($\kappa=0.773$) and human evalutors ($\kappa=0.684$) also further substantiates the high level of alignment in evaluation between LLM judges and human evaluators. Overall, These findings suggests that LLMs can serve as effective assistants for preliminary UML quality assessment, reducing the cognitive and time burden on human reviewers. However, due to their limited contextual understanding, final validation should remain human-guided, particularly for domain-intensive models. 

Future advancements in LLM capabilities could enable them to effectively assist requirement engineers (REs) in the co-design of UML diagrams. LLMs could interactively engage with users by asking clarifying questions, refining designs iteratively, and ensuring alignment with system requirements. This collaborative approach accelerates the overall diagram generation process. Leveraging LLMs for model evaluation could also substantially reduce the time and effort required for human review while maintaining scalable and high-quality assessment standards. A human-AI collaborative framework offers a promising direction, combining LLM efficiency with human expertise to enhance both the accuracy and reliability of UML model development.

% The results shown in Table \ref{tab:stats-cohend-HITL} differ significantly from previous study \cite{ferrari2024model}, likely due to differences in dataset scale and model diversity. Whereas the prior study evaluated GPT-3.5 on UML sequence diagram generation using five criteria, this study incorporates multiple LLMs for UML class diagram generation. Consequently, the performance of the best-performing model in this context naturally affects the degree of alignment with earlier research.

% A notable limitation arises from the use of researchers themselves as human evaluators, without the involvement of domain experts. This human-in-the-loop setup introduces potential bias and subjective judgment, especially when evaluators lack specialized domain knowledge. Hence, while human evaluators demonstrated general consistency, future studies should engage domain experts to improve the validity and reliability of UML evaluation outcomes and strengthen the interpretability of LLM-based judgments in SE design contexts.

% how bias and errors have been addressed
% To minimise bias during model evaluation, two external judges distinct from the evaluated models were selected. Identical evaluation criteria were applied to both human evaluators and LLM judges, and model identities were anonymised to prevent biased judgements. The memory functions of the evaluated models were also disabled to avoid memory-induced hallucination from prior sessions. 
% During the model generation, occasional inconsistencies between model outputs and requirements were observed, likely due to the inclusion of real-world UML examples in the prompts, which sometimes led to misinterpretation. While most models required a single prompt, others, such as Llama 3.1 model, needed multiple iterations to produce accurate diagrams. These iterative refinements helped reduce output errors and improve alignment with complex requirements, thus enhancing the overall accuracy of the model generation process. 


% need to relate results back to previous study
% Our findings align with the previous study \cite{ferrari2024model}, which demonstrated that LLM-based design evaluations can capture semantic quality effectively. Instead of generating UML sequence diagrams using an LLM, this study was further extended by incorporating multiple LLMs in UML class diagrams generation, and utilising \textit{LLM-as-a-Judge} approach \cite{dhurandhar-etal-2024-ranking}, \cite{liusie2023llm} in the evaluation in addition to human evaluators.



==> source/kappa_table.tex <==
\begin{table}[h!]
\centering
\label{tab:pariwsie-cohen-kappa-ALL}
\caption{Pairwise Cohen's Kappa between all evaluators (LLM judges and HITL)}
\begin{tabular}{lcccc}
\toprule
\textbf{Evaluator} & \textbf{Grok} & \textbf{Mistral} & \textbf{A1} & \textbf{A2} \\
\midrule
Grok     & 1.0000 & 0.7727 & 0.4737 & 0.4118 \\
Mistral  & 0.7727 & 1.0000 & 0.6250 & 0.5455 \\
A1       & 0.4737 & 0.6250 & 1.0000 & 0.6842 \\
A2       & 0.4118 & 0.5455 & 0.6842 & 1.0000 \\
\bottomrule
\end{tabular}
\label{tab:pairwise-kappa}
\end{table}


==> source/tables/tab-five-criteria-human331.tex <==
\begin{table}[H]
\caption{5-criteria evaluation of \textbf{ChatGPT GPT-5} UML diagrams across All Datasets Judged Independent evaluators (A1 and A2)}

\centering
\begin{tabular}{|l|c|c|c|c|c|c|}
\hline
\textbf{Dataset} & \textbf{Comp.} & \textbf{Corr.} & \textbf{Stand.} & \textbf{Underst.} & \textbf{Term.} & \textbf{Total} \\
\hline
g14-datahub         & 5  & 4      & 4   & 5   & 5    & 23 \\
g04-recycl.    & 4  & 4    &  5    & 4   & 5    &   22 \\
g02-camper.     & 4    & 4    &  4  & 4     &   4  &   20\\
UHOPE               &  4   & 5     & 5   &  5  & 5    &   24 \\
autopilot           &4   & 4    &  4    & 4   &4     &   20 \\
Finite State.       & 4    &  4     &    5  & 3     & 4    &   20 \\
Inventory           & 4    &  4     &  4    & 4     &4     &  20 \\
Pacemaker           & 3  & 3      &   3 & 3     & 3    &  15\\
\hline
\end{tabular}
\end{table}


==> source/tables/tab-fivecriteria-data1.tex <==

\begin{table}[H]
\caption{5-criteria evaluation of \textbf{GPT-5} across all datasets judged by Grok}
\label{tab:fivecriteria-grok}
\centering
\begin{tabular}{|l|c|c|c|c|c|c|}
\hline
\textbf{Dataset} & \textbf{C1} & \textbf{C2} & \textbf{C3} & \textbf{C4} & \textbf{C5} & \textbf{Total} \\
\hline
g14-datahub         & 5 & 4 & 5 & 5 & 5 & 24 \\
g04-recycl.       & 5  & 5  &  5   & 5  & 5    &   25 \\
g12-camper.     & 4  & 3  &  3   & 3  &   5  &   18 \\
UHOPE               &  5 & 5  & 5    &  5 & 5    &   25 \\
autopilot           &  5 & 5  &  5   &5   &5     &   25 \\
FiniteState.  & 4  &  4 &    5 & 4  & 5    &   22 \\
Inventory           & 4  &  4 &  5   & 4  &5     &  22  \\
Pacemaker           & 2  & 3  &   3  & 4  & 5    &  17  \\
\hline
\end{tabular}
\vspace*{0.1em}
\\ *C1 = Completeness, C2 = Correctness, C3 = Adherence to Standards, C4 = Comprehensibility, C5 = Terminological alignment
\end{table}


==> source/tables/tab-fivecriteria-data2.tex <==
\begin{table}[H]
\caption{5-criteria evaluation of \textbf{GPT-5} across All Datasets Judged by Mistral}
\label{tab:fivecriteria-mistral}
\centering
\begin{tabular}{|l|c|c|c|c|c|c|}
\hline
\textbf{Dataset} & \textbf{C1} & \textbf{C2} & \textbf{C3} & \textbf{C4} & \textbf{C5} & \textbf{Total} \\
\hline
g14-datahub         & 4 & 4 & 4 & 4 & 4 & 20 \\
g04-recycl.      & 4  & 4  &  5   & 4  & 4    &   21 \\
g12-camper.     & 4  & 4  &  4   & 3  &   4  &   19 \\
UHOPE               &  5 & 5  & 4    &  4 & 4    &   22 \\
autopilot           &  4 & 4  &  4   & 4  &4     &   20 \\
FiniteState. & 4  &  4 &    5 & 4  & 4    &   21 \\
Inventory           & 4  &  4 &  5   & 4  &4     &  21  \\
Pacemaker           & 3  & 3  &   3  & 4  & 4    &  17  \\
\hline
\end{tabular}
\end{table}


==> source/tables/tab-fivecriteria-data3.tex <==
\begin{table}[H]
\caption{5-criteria evaluation of \textbf{GPT-5} UML diagrams across all datasets judged by independent evaluator A1}
\centering
\label{tab:fivecriteria-a1}
\begin{tabular}{|l|c|c|c|c|c|c|}
\hline
\textbf{Dataset} & \textbf{C1} & \textbf{C2} & \textbf{C3} & \textbf{C4} & \textbf{C5} & \textbf{Total} \\
\hline
g14-datahub             & 4 & 4 & 4 & 4 & 5 & 21 \\
g04-recycl.            & 4 & 4 & 5 & 4 & 5 & 22 \\
g12-camper.          & 4 & 4 & 4 & 4 & 5 & 21 \\
UHOPE                  & 4 & 4 & 4 & 5 & 5 & 22 \\
autopilot          & 3 & 4 & 4 & 5 & 5 & 21 \\
FiniteState.   & 4 & 4 & 5 & 5 & 4 & 22 \\
Inventory              & 4 & 4 & 5 & 4 & 5 & 22 \\
Pacemaker              & 3 & 3 & 3 & 3 & 4 & 16 \\
\hline
\end{tabular}
\end{table}


==> source/tables/tab-fivecriteria-data4.tex <==
\begin{table}[H]
\caption{5-criteria evaluation of \textbf{GPT-5} UML diagrams across all datasets judged by independent evaluator A2}
\centering
\label{tab:fivecriteria-a2}
\begin{tabular}{|l|c|c|c|c|c|c|}
\hline
\textbf{Dataset} & \textbf{C1} & \textbf{C2} & \textbf{C3} & \textbf{C4} & \textbf{C5} & \textbf{Total} \\
\hline
g14-datahub               & 5 & 4 & 4 & 5 & 5 & 23 \\
g04-recycl.           & 4 & 4 & 5 & 4 & 5 & 22 \\
g12-camper.            & 4 & 4 & 4 & 4 & 5 & 21 \\
UHOPE                  & 4 & 5 & 5 & 5 & 5 & 24 \\
autopilot             & 4 & 4 & 4 & 4 & 4 & 20 \\
FiniteState.   & 4 & 4 & 5 & 3 & 4 & 20 \\
Inventory              & 4 & 4 & 4 & 4 & 4 & 20 \\
Pacemaker              & 3 & 3 & 3 & 3 & 3 & 15 \\
\hline
\end{tabular}
\end{table}


==> source/tables/tab-fivecriteria-stats.tex <==
\begin{table}[H]
\caption{Statistics and test results from LLM judges}
\label{tab:stats-cohend}
\centering
\begin{tabular}{|l|c|c|c|c|}
\hline
\textbf{Criterion} & \textbf{Mean}  & \textbf{Cohen's d} & \textbf{Eff. S.} \\
\hline
Completeness     &4.125    &  0.30 & small\\
Correctness      &4.062       &  0.18  & none \\
Standards        & 4.375   & 0.30&  small\\
Understanding      &  4.125& 0.86 & large\\
Terminology      &    4.50 & inf  &  large\\
\hline
\end{tabular}
\end{table}


==> source/tables/tab-geminihuman.tex <==
% \begin{table}[t]
\begin{table}[H]
\caption{Example Rank comparison between \textbf{Gemini’s 2.0 Flash thinking} and independent researcher evaluation ranking}
\label{tab:rank-comparison}
\centering
\begin{tabular}{|l|c|c|c|c|}
\hline
\textbf{Dataset} & \textbf{Gemini Rank} & \textbf{Human Rank} & \textbf{d} & \textbf{d\textsuperscript{2}} \\
\hline
% g14-datahub         & 1 & 1 & 0  & 0 \\
% g04-recycling       & 1 & 1 & 0  & 0 \\
% g02-camperplus      & 2 & 1 & 1  & 1 \\
% UHOPE               & 2 & 2 & 0  & 0 \\
% autopilot           & 2 & 3 & -1 & 1 \\
% Finite State Machine & 3 & 2 & 1  & 1 \\
% Inventory           &   &   &    &   \\
% Pacemaker           &   &   &    &   \\
g14-datahub         &  &  &   &  \\
g04-recycling       &  &  &   &  \\
g02-camperplus      &  &  &   &  \\
UHOPE               &  &  &   &  \\
autopilot           &  &  &  &  \\
Finite State Machine & &  &   &  \\
Inventory           &   &   &    &   \\
Pacemaker           &   &   &    &   \\
\hline
\multicolumn{4}{|r|}{\textbf{Sum =}} & 3 \\
\hline
\end{tabular}
\end{table}


==> source/tables/tab-rankings-grok.tex <==
\begin{table}[H]
\caption{LLM Rankings per Dataset judged by \textbf{Grok} (1) and Mistral (2)}
\label{tab:llm-rankings-grok}
\centering
\begin{tabular}{|l|c|c|c|c|}
\hline
\textbf{Dataset \rev{(1)}} & \textbf{ChatGPT} & \textbf{Claude} & \textbf{Gemini} & \textbf{Llama} \\
\hline
g14-datahub                & 1 &2  & 3 & 4  \\
g04-recycling              &  2&1  &  3&  4 \\
g12-camperplus             &  3&1  &  2&   4\\
UHOPE                      &  2&1  &  3&   4\\
autopilot                  &  1&2  &  3&   4\\
FiniteStateMachine       &  1&2  &  3&   4\\
Inventory                  &  1 &2   & 3  & 4  \\
Pacemaker                  &  1 & 2  & 3  &  4 \\
\hline
\end{tabular}

\vspace*{0.5em}
\begin{tabular}{|l|c|c|c|c|}
\hline
\textbf{Dataset \rev{(2)}} & \textbf{ChatGPT} & \textbf{Claude} & \textbf{Gemini} & \textbf{Llama} \\
\hline

g14-datahub                & 1 &3  & 2 & 4  \\
g04-recycling              &  2&1  &  3&  4 \\
g12-camperplus             &  3&1  &  2&   4\\
UHOPE                      &  1&2  &  3&   4\\
autopilot                  &  1&2  &  3&   4\\
FiniteStateMachine         &  2&1  &  3&   4\\
Inventory                  &  1 &2   & 3  & 4  \\
Pacemaker                  &  3 & 1  & 2  &  4 \\
\hline
\end{tabular}

\end{table}




==> source/tables/tab-rankings-mistral.tex <==
\begin{table}[H]
\caption{LLM Rankings per Dataset judged by \textbf{Mistral}}
\label{tab:llm-rankings}
\centering
\begin{tabular}{|l|c|c|c|c|}
\hline
\textbf{Dataset} & \textbf{ChatGPT} & \textbf{Claude} & \textbf{Gemini} & \textbf{Llama} \\
\hline

g14-datahub                & 1 &3  & 2 & 4  \\
g04-recycling              &  2&1  &  3&  4 \\
g12-camperplus             &  3&1  &  2&   4\\
UHOPE                      &  1&2  &  3&   4\\
autopilot                  &  1&2  &  3&   4\\
FiniteStateMachine         &  2&1  &  3&   4\\
Inventory                  &  1 &2   & 3  & 4  \\
Pacemaker                  &  3 & 1  & 2  &  4 \\
\hline
\end{tabular}

\end{table}

